Enhanced Renewable Energy Forecasting and Operations through Probabilistic Forecast Aggregation

Accurate and reliable forecasting of renewable energy generation is crucial for the efficient integration of renewable sources into the power grid. In particular, probabilistic forecasts are becoming essential for managing the intrinsic variability and uncertainty of renewable energy production, especially wind and solar generation. This paper considers the setting where probabilistic forecasts are provided for individual renewable energy sites using, e.g., quantile regression models, but without any correlation information between sites. This setting is common if, e.g., such forecasts are provided by each individual site, or by multiple vendors. However, to effectively manage a fleet of renewable generators, it is necessary to aggregate these individual forecasts to the fleet level, while ensuring that the aggregated probabilistic forecast is statistically consistent and reliable. To address this challenge, this paper presents the integrated use of Copula and Monte-Carlo methods to aggregate individual probabilistic forecasts into a statistically calibrated, probabilistic forecast at the fleet level. The proposed framework is validated using synthetic data from several large-scale systems in the United States. This work has important implications for grid operators and energy planners, providing them with better tools to manage the variability and uncertainty inherent in renewable energy production.

==> tex/review.tex <==
\section{Literature Review}
\label{sec:literature_review}



Time series forecasting in power systems has been extensively studied, with methods evolving from traditional statistical models such as ARIMA \cite{miswan2016arima,alberg2018short} to machine learning approaches like support vector regression \cite{zahid2019electricity}, quantile regression forests \cite{8272993,he2020day}, and advanced deep learning techniques \cite{8863951,amarasinghe2017deep}. The increasing integration of renewable energy resources (RES) has shifted the focus toward high-dimensional probabilistic forecasting, which captures interdependencies between different targets and provides uncertainty-aware solutions for improved decision-making.

A key challenge in power system forecasting is the need for coherent forecasts across different levels of aggregation, including site, zone, and system levels. Ensuring that aggregated probabilistic forecasts remain valid and maintain consistency across hierarchical levels is essential for reliable grid operations.

Several methodologies have been developed to address the probabilistic forecast aggregation problem. \cite{taieb2021hierarchical} proposes an empirical copula-based bottom-up procedure, where the marginal predictive distributions at each node are used to estimate the joint distribution via an empirical copula, ensuring coherence in the aggregated forecasts. Similarly, \cite{sun2019conditional} introduces a clustering-based approach for wind farms, reducing computational costs before employing a copula-based method to capture inter-cluster dependencies. Additionally, \cite{taieb2017coherent} models the dependency structure using a copula framework, enabling the computation of a coherent summation distribution from marginal predictive distributions.








